A first-order logic for string diagrams

Equational reasoning with string diagrams provides an intuitive means of proving equations between morphisms in a symmetric monoidal category. This can be extended to proofs of infinite families of equations using a simple graphical syntax called !-box notation. While this does greatly increase the proving power of string diagrams, previous attempts to go beyond equational reasoning have been largely ad hoc, owing to the lack of a suitable logical framework for diagrammatic proofs involving !-boxes. In this paper, we extend equational reasoning with !-boxes to a fully-fledged first order logic called with conjunction, implication, and universal quantification over !-boxes. This logic, called !L, is then rich enough to properly formalise an induction principle for !-boxes. We then build a standard model for !L and give an example proof of a theorem for non-commutative bialgebras using !L, which is unobtainable by equational reasoning alone.

==> old.tex <==
For a definition of tensor expressions and equivalence of such expressions look at~\cite{NoncommBB}.

To define a theory we need to decide what diagrams are valid. This is done similarly to mathematical logic where a signature describes the non-logical symbols of a formal language, from which we can build more complex formulas. For our diagrammatic purposes a \textit{signature} $\Sigma$ is made up of a pair $(\mathcal{O},\mathcal{M})$. The set of Object types $\mathcal{O}$ lists the types which can be assigned to edges. Since our edges are directed, we need to refer to inputs and outputs of each type seperately. For $A\in\mathcal{O}$ we write $\ein{A}$ for an input of type $A$, $\eout{A}$ for an output of type $A$ and $\mathcal{O'}$ for the set of edge types with direction, $\mathcal{O'} :=\{\ein{A},\eout{A} | A\in\mathcal{O}\}$. The set of Morphisms $\mathcal{M}$ is made up of morphisms from the identity object $I$ to tensor products in $\mathcal{O'}$. i.e. $\phi:I\rightarrow X_1 \otimes X_2 \otimes \ldots \otimes X_n$, for $X_1,\ldots,X_n\in\mathcal{O'}$.

Graphically a morphism can be represented as a circular node with a tick to define the start, then edges clockwise labelled by their type.


\subsection{Diagrammatic theories}\label{sub:diagrammatic_theories}

A \textit{Diagrammatic theory} is made up of a signature $\Sigma$ and a set of \textit{Diagrammatic equations} $E$. $E$ contains equalities between diagrams. For an equality between to diagrams to be valid they must have the same \textit{boundaries}, i.e. the same free edges. 

One common example is the theory of commutative frobenius algebras. Its signature can be written as:
\[\Sigma:= \big( \{X\}, \{ \mu:I\rightarrow X\otimes X^*\otimes X^*, \eta:I\rightarrow X, \delta:I\rightarrow X\otimes X\otimes X^*, \epsilon:I\rightarrow X^* \} \big) \]
In this case morphism names can be dropped as each is uniquely determined by its arity. Hence we can now write this signature graphically as:
\[ \Sigma \ =\  \tikzfig{frob_sig} \]

% The following are examples of valid diagrams for this signature.

% \ctikzfig{comm_frob_egs}

For the diagrammatic equations we have:
\begin{equation}
  \tikzfig{comm_frob_eqns}
\end{equation}
i.e (co)associativity, (co)unit, (co)commutativity and the frobenius law.

A \textit{model} of a diagrammatic theory $(\Sigma,E)$ is an assignment of an explicit morphism (of the prescribed arity) to every generator in $\Sigma$ such that each equation in $E$ holds.

Models allow us to assign morphism to any diagram in our signature. We can then check whether two diagrams are equal in this model by determining whether they represent the same morphism. Two diagrams are considered to be equal in a diagrammatic theory if they are equal under any possible model of the theory.



\subsection{!-Boxes}\label{sub:!-boxes}

In many cases a theory can be simplified by defining variable arity nodes to replace many fixed arity nodes. This is true of the commutative frobenius algebra example above. All nodes in the signature can be replaced by one `spider' node with variable number of inputs and outputs. The diagrammatic equations are then replaced by just two `families' of equations. Our theory can now be presented as:
\[
\Sigma' \ =\ \left\{ \ \tikzfig{spider} \ \right\} \qquad
E' \ =\ \left\{ \ \tikzfig{spider_merge}, \ \ \ \
                        \tikzfig{spider_elim} \ \right\}
\]

These new families of equations have dots to represent that a part of the diagram can appear multiple times. To make this more rigorous \textit{!-boxes} (pronounced bang-boxes) were introduced in~\cite{DixonDuncan2009} as a way to define which sections can be repeated. !-Boxes were then formalised and used in~\cite{PatternGraph,KissingerThesis,MerryThesis} and the graphical proof assistant Quantomatic~\cite{Quantomatic} was developed to automate reasoning with !-boxes in commutative graphical systems. We draw a rectangle around part of a diagram to denote that it can be copied any number of times. There are then two operations on !-boxes which combined allow us to retrieve all concrete diagrams represented by it. These are $\Kill_B$ which removes the !-box $B$ with all contents and $\Exp_B$ which creates a copy of the contents of the !-box $B$ and attaches it to the same nodes as the original.

Since we are not assuming edges on nodes commute we need to be specific about where new edges from $\Exp$ operations get added. We do this by choosing an expansion direction for sets of adjacent edges from a node which enter a !-box. The direction is marked on diagrams as an arc over the edges. Equations between !-box diagrams require that they have the same free edges in the same !-boxes (called having the same boundary). For example, our informal theory above can be replaced by the !-box version. 

\[
\Sigma' \ =\ \left\{ \ \tikzfig{spider_bb} \ \right\} \qquad
E' \ =\ \left\{ \ \tikzfig{spider_merge_bb}, \ \
                        \tikzfig{spider_elim} \ \right\}
\]

For our tensor notation we enclose the nodes inside a !-box $B$ in square brackets with a superscript label, $[\ldots]^B$. Similarly we need edges entering a !-box to be annotated with their expansion direction. We surround clockwise expanding edges in $\rexp{\ldots}^B$ and anticlockwise expanding edges in $\lexp{\ldots}^B$.

We refer to expressions in the adapted tensor notation as !-tensor expressions. Here are a few examples of !-tensor expressions and the diagrams they represent.
\begin{center}
\(
\begin{matrix}
  \psi_{\+a' \<b' \lexp{\+a \<b}^A} []^A & &
  \psi_{\rexp{\+a \<b}^A \+a' \<b'}[]^A & &
  \psi_{\rexp{\+a}^A \+a' \rexp{\<b}^A \<b'}[]^A \\
  & & & & & \\
  \tikzfig{expand-order1} &
  \quad\textrm{vs.}\quad &
  \tikzfig{expand-order2} &
  \quad\textrm{vs.}\quad &
  \tikzfig{expand-order3}
\end{matrix}
\)
\end{center}

We allow !-boxes to be nested inside of other !-boxes. Expanding the parent !-box creates a (freshly named) copy of the child !-box along with the rest of its contents. Similarly, edge groups must be nested if the edges enter more than one !-box. In the diagram below we have a !-tensor with nested !-boxes.
\begin{center}
\(
\phi_{\+a \lexp{ \lexp{\<b}^B }^A} [[\phi_{\+b\<c}]^B]^A \ :=\
\tikzfig{nested-ex}
\)
\end{center}

Note that we have labelled each arc with its associated !-box. This is not necessary as we adopt the convention that arcs corresponding to a !-box $B$ are always drawn \textit{closer} to the node than arcs for children of $B$.

Next we present the formal definitions for our !-tensor language and state some of the important facts about it. For a complete rigorous treatment of !-tensors look at~\cite{NoncommBB}.


\subsection{!-Tensors}\label{sub:!tensors}

\begin{definition}\label{def:edgeterm-equiv}
Fix disjoint, infinite sets $\edgenames$ and $\boxnames$ of edge names and !-box names, respectively. The set of \textit{edgeterms} $\edgeterms$ is defined recursively as follows:
  \begin{align*}
    \bullet\; &\epsilon \in \edgeterms && \text{(empty edgeterm)} \\
    \bullet\; & \ein a, \eout a \in \edgeterms && a \in \edgenames \\
    \bullet\; &\rexp{e}^A,\rexp{e}^A \in \edgeterms && e\in\edgeterms,\; A\in\boxnames \\
    \bullet\; & e f \in \edgeterms && e,f\in\edgeterms
  \end{align*}
  % Two edgeterms are equivalent if one can be transformed into the other by:
  % \begin{equation}\label{eqn:edgeterm_equiv}
  %   e(fg) \equiv (ef)g \qquad
  %   \epsilon e \equiv e \equiv e \epsilon \qquad
  %   \term{[\epsilon>A} \equiv \epsilon \equiv \term{<\epsilon]A}
  % \end{equation}
  % The first two represent associativity and identity of concatenation, with $\epsilon$ as the unit. The last equivalence says that empty edge groups can be ignored.
\end{definition}

Since the well-formedness conditions for !-tensor expressions are a bit more complicated than for tensor expressions, we first define the set of all !-pretensor expressions, including those that may be ill-formed.

Letting $1$ represent the empty !-tensor and $1_{\+a\<b}$ represents an identity edge with input named $b$ and output named $a$ we can define !-tensor expressions.

\begin{definition}\label{def:!-tensors}
The set of all !-tensor expressions $\sgraphterms$ for a signature $\Sigma$ is defined recursively as:
  \begin{align*}
    \bullet\; &1, 1_{\+a\<b} \in \sgraphterms && a,b\in\edgenames\\
    \bullet\; &\phi_{e} \in \sgraphterms && e\in\edgeterms, \phi\in\Sigma \\
    \bullet\; &[G]^A \in \sgraphterms && G\in\sgraphterms, \; A\in\boxnames \\
    \bullet\; & G H \in \sgraphterms && G,H\in\sgraphterms
  \end{align*}
  Under certain well-formedness conditions to ensure that no !-box/edge names appear more than once and bound edge names are compatible.
\end{definition}

We introduce the notion of a \textit{context}, which lists the !-boxes in which a certain edge name occurs, from the inside-out. These come in two flavours, \textit{edge contexts} and \textit{node contexts}.

\begin{definition}
  Given a directed edge $a$ in a !-tensor $G$ nested as $\term{[[\phi.<<a>{E_1}\ldots>{E_n}.]{N_1}\ldots]{N_m}}$.

  We define the \textit{edge context}, \textit{node context}, and \textit{context} of $a$ respectively as:
    \begin{align*}
      \ectx_G(a)&:=[E_1,\ldots,E_n] && \text{(edge context)} \\
      \nctx_G(a)&:=[N_1,\ldots,N_m] && \text{(node context)} \\
      \ctx_G(a)&:=\ectx_G(a).\nctx_G(a) && \text{(context)}
    \end{align*}
    That is, $\ectx_G(a)$ lists the !-boxes containing $a$ that occur as part of $a$'s edgeterm, and $\nctx_G(a)$ lists the rest. 
\end{definition}

Finally, a !-tensor expression is a !-pretensor expression where !-box/edge names must be suitably unique and occur in compatible contexts:

\begin{definition}\label{def:tensor_conditions}
  A !-tensor expression is a !-pretensor expression satisfying the following conditions:
  \begin{itemize}
    \item[F1.] $\ein a$ and $\eout a$ occur at most once for each edge name $a$
    \item[F2.] $\term{[\ldots]A}$ must occur at most once for each !-box name $A$
    \item[C1.] $\ectx_G(a)\cap \nctx_G(a)=\varnothing$ \: for all edges $a \in \edgenames$ in $G$
    \item[C2.] If $\ectx_G(a)=[B_1,\ldots,B_n]$ \; then all $B_i\in\Boxes(G)\:$ and $\; B_1\prec_G B_2\prec_G \ldots \prec_G B_n$
    \item[C3.] For all bound pairs $\ein a, \eout a$ of edge names in $G$, there exist lists $es, bs$ of !-box names such that:
    \[ es.\nctx_G(\ein{a}) = \ectx_G(\eout{a}).bs
       \quad \textrm{and} \quad
       es.\nctx_G(\eout{a}) = \ectx_G(\ein{a}).bs \]
  \end{itemize}
  where $A \prec_G B$ means that the !-box $A$ is nested immediately inside $B$ in $G$ (i.e.~without other !-boxes nested between). We write $\graphterms$ for the set of all !-tensor expressions for a signature $\Sigma$.
\end{definition}

As with the standard tensor case, two !-tensor expressions may represent the same diagram, in which case we say the expressions are equivalent.  










\subsection{Quantification}\label{sub:quantification}

% $A\childof B$
% $A\descof B$
% $A\childin{G'} B$
% $A\descin{\Exp(G)} B$
% $\children{A}$
% $\downset{A}$
% $\parents{A}$
% $\upset{A}$
% $\updownset{A}$
% $\components{X}$x
% $\topboxes{X}$
% $\quant{A}X$


\TODO{Change this to reference `FIX' instead. More obviously a hack this way. :)}
The previous standard for diagrammatic equational reasoning was the idea of substitution. An equation $G=H$ would mean that any time $G$ appeared somewhere, it could be `taken out' and then `replaced by' $H$. In this paper we wish to replace this by a natural deduction system in which new equations are deduced from old by logical rules. Since a !-tensor equation represents countably many concrete diagram equations (with $Kill$, $Exp$ playing the role of the recursive definition), a logical idea would then be to try to prove such families of rules using induction. Induction can be written as a logical rule in the form:
\[
  \AxiomC{$\Kill_A(X)$}
  \AxiomC{$X\rightarrow_A\Exp_A(X)$}
  \RightLabel{\scriptsize($Induct_A$)}
  \BinaryInfC{$X$}
  \DisplayProof
\]
Where by $\rightarrow_A$ we mean implication in which the !-box $A$ is effectively fixed~\cite{MerryThesis}. Else we would trivially be allowed to expand $A$ making the sentence a tautology. There are also possibly new !-boxes introduced by expanding $A$ which may or may not need induction to prove. To remove this ambiguity we need to explicitly state when a !-box is quantified over (meaning !-box operations are allowed). This becomes particularly important when we have nesting of !-boxes (a !-box inside another must be copied along with the other contents, but a new fresh name must be assigned to all free !-boxes and edges).

When we only have one !-box, $A$, in an equation $G=H$, we have an intuition as to what it means to say $\forall A (G=H)$. Namely that any concrete equation coming from $G=H$ (i.e $\Kill_A\Exp_A^n(G=H)$ for any $n\in\mathbb{N}$) is true. The trouble comes when attempting to quantify over a !-box with nesting. For example saying $\forall B (G=H)$ doesn't make sense when $B$ is nested inside a !-box $A$. The quantification over $B$ is referencing a !-box which will have copies made (during $\Exp_A$) then will be killed. To remove this ambiguity we will not quantify over single !-boxes. We will instead need to quantify over all !-boxes in some component of the !-box structure. In other words, to quantify over a !-box every child and parent must be quantified over at the same time.

Take for example an equation containing !-boxes $A,B,C,D$ where $B$ and $C$ are nested in $A$, by representing `$B$ is a child of $A$' by a line from $A$ down to $B$, we can draw this as:
\begin{forest}
[A
  [B]
  [C]
]
\end{forest}
\begin{forest}
[D]
\end{forest}

We can then quantify over either of the two trees (or both), i.e $\{A,B,C\}$ or $\{D\}$. Quantifying over $\{A,B,C\}$ signifies that $X$ is true after any !-box operations on $A,B,C$ and their copies, where they are eventually all killed. Note we still need to instantiate $D$ to get to a concrete proposition.

To deal with nested !-boxes, we introduce some basic order-theoretic notions.




\subsection{Formulas}\label{sub:formulas}

% As seen in section \ref{sub:diagrammatic_theories}, diagrammatic theories are pairs $(\Sigma,E)$ where $\Sigma$ is the signature and $E$ is a (possibly infinite) set of diagrammatic equations. We wish to recursively define the valid formulas for signature $\Sigma$. Whether a formula is true or not may then be provable from $E$.

% \begin{definition}
%   Two !-box structures are said to be disjoint if their connected components are disjoint sets of !-boxes.
% \end{definition}


% If we have nesting then the proof that $X\vdash\Exp_{B}(X)$ may involve induction on the fresh copies of children of $B$.

\subsection{Renaming}\label{sub:renaming}

In a formula $X$ any !-box which is quantified over is bound and so its name is unimportant. Hence $\quant{A}X=\forall\downset{A}[B\mapsto B'].X[B\mapsto B']$. This can easily be shown from existing rules. Letting $\rn$ choose globally fresh names for $\downset{A}$:
\[
  \AxiomC{$\Gamma \vdash \quant{A}X$}
  \RightLabel{\scriptsize$(\forall E)$}
  \UnaryInfC{$\Gamma \vdash \rn(X)$}
  \RightLabel{\scriptsize$(\forall I)$}
  \UnaryInfC{$\Gamma \vdash \forall\downset{A}[B\mapsto B'].X[B\mapsto B']$}
  \DisplayProof
\]

%? Explain renaming of non-bound !-boxes globally

To form compositions of rules concatenating free edges we need to be able to rename free edges. We might think this means introducing a new rule, but it turns out this can be derived from the existing rules. We write $G[a\mapsto b]$ for $G$ with edge $a$ replaced by $b$

\begin{lemma}\label{lem:edge_renamer}
  \[
    \AxiomC{$\Gamma \vdash G = H$}
    \RightLabel{\rm\scriptsize(EdgeRename)}
    \UnaryInfC{$\Gamma \vdash (G = H)[a\mapsto b]$}
    \DisplayProof
  \]
  Where the edge $a$ is free in $G$ (and therefore also in $H$) and $b$ does not appear in $G$ or $H$.
\end{lemma}
\begin{proof}
  Without loss of generality we take the case where $a$ is an output in $G,H$. \\
  If $a$ is not contained in a any !-box then the proof can be derived from (Prod):
  \[
    \AxiomC{$\Gamma \vdash G = H$}
    \RightLabel{\scriptsize(Prod)}
    \UnaryInfC{$\Gamma \vdash G 1_{ab} = H 1_{ab}$}
    \RightLabel{\scriptsize($\equiv$)}
    \UnaryInfC{$\Gamma \vdash (G = H)[a\mapsto b]$}
    \DisplayProof
  \]
  Where $1_{ab}$ is an identity edge going from input $a$ to output $b$. \\
  Otherwise let $B$ be the (lowest level) !-box containing $a$. Then using (Weak):
  \[
    \AxiomC{$G = H$}
    \RightLabel{\scriptsize(Weak)}
    \UnaryInfC{$\Wk{B}{1_{ab}}(G) = \Wk{B}{1_{ab}}(H)$}
    \RightLabel{\scriptsize($\equiv$)}
    \UnaryInfC{$G[a\mapsto b] = H[a\mapsto b]$}
    \DisplayProof
  \]
\end{proof}

\begin{theorem}\label{thm:edge_renamer}
  \[
    \AxiomC{$\Gamma \vdash Z$}
    \RightLabel{\rm\scriptsize(Rename)}
    \UnaryInfC{$\Gamma \vdash Z[a\mapsto b]$}
    \DisplayProof 
  \]
  Where the edge $a$ is free in $G$ (and therefore also in $H$) and $b$ does not appear in $Z$.
\end{theorem}
\begin{proof}
  We proceed by structural induction on the definition of the formula $Z$, which gives us four cases to check.
  \begin{itemize}
    \item $(G=H)$ \\
      This case is exactly Lemma~\ref{lem:edge_renamer}.
    \item $X\wedge Y$
      \[
        \AxiomC{$\Gamma \vdash X\wedge Y$}
        \RightLabel{\scriptsize ($\wedge E_1$)}
        \UnaryInfC{$\Gamma \vdash X$}
        \RightLabel{\scriptsize (IH)}
        \UnaryInfC{$\Gamma \vdash X[a\mapsto b]$}
        \AxiomC{$\Gamma \vdash X\wedge Y$}
        \RightLabel{\scriptsize ($\wedge E_2$)}
        \UnaryInfC{$\Gamma \vdash Y$}
        \RightLabel{\scriptsize (IH)}
        \UnaryInfC{$\Gamma \vdash Y[a\mapsto b]$}
        \RightLabel{\scriptsize ($\wedge I$)}
        \BinaryInfC{$\Gamma \vdash (X\wedge Y)[a\mapsto b]$}
        \DisplayProof
      \]
    \item $X\rightarrow Y$
      \[
        \AxiomC{$X[a\mapsto b] \vdash X[a\mapsto b]$}
        \RightLabel{\scriptsize (IH)}
        \UnaryInfC{$X[a\mapsto b] \vdash X$}
        \AxiomC{$\Gamma \vdash X\rightarrow Y$}
        \RightLabel{\scriptsize ($\rightarrow E$)}
        \UnaryInfC{$\Gamma, X \vdash Y$}
        \RightLabel{\scriptsize (IH)}
        \UnaryInfC{$\Gamma, X \vdash Y[a\mapsto b]$}
        \RightLabel{\scriptsize ($\wedge I$)}
        \BinaryInfC{$\Gamma, X[a\mapsto b] \vdash Y[a\mapsto b]$}
        \RightLabel{\scriptsize ($\wedge I$)}
        \UnaryInfC{$\Gamma \vdash (X\rightarrow Y)[a\mapsto b]$}
        \DisplayProof
      \]
      The inductive hypothesis applied on the left is valid since $b$ is not in $X$ so it is free in $X[a\mapsto b]$.
    \item $\quant{A}X$
      \[
        \AxiomC{$\Gamma \vdash \quant{A}X$}
        \RightLabel{\scriptsize ($\forall E$)}
        \UnaryInfC{$\Gamma \vdash \rn(X)$}
        \RightLabel{\scriptsize (IH)}
        \UnaryInfC{$\Gamma \vdash \rn(X)[a\mapsto b]$}
        \RightLabel{\scriptsize ($\equiv$)}
        \UnaryInfC{$\Gamma \vdash \rn(X[a\mapsto b])$}
        \RightLabel{\scriptsize ($\forall I$)}
        \UnaryInfC{$\Gamma \vdash (\quant{A}X)[a\mapsto b]$}
        \DisplayProof
      \]
      Where $\rn$ chooses fresh names for the !-boxes in $\downset{A}$.
  \end{itemize}
\end{proof}

By iterating this rule, we can rename using any function $\rn:\edgenames\rightarrow\edgenames$ with finite support (i.e $\rn(x)=x$ for all but finitely many $x$).
We write $X[\rn]$ for $X$ with $\rn$ applied to all free edge names. Then, from Theorem~\ref{thm:edge_renamer}, it follows that:
\begin{equation}\label{eq:renamer'}
  \AxiomC{$\Gamma \vdash X$}
  \RightLabel{\rm\scriptsize(Rename')}
  \UnaryInfC{$\Gamma \vdash X[\rn]$}
  \DisplayProof
\end{equation}

% We do this with a renaming function $\rn$ which replaces some free !-box/edge name with a fresh !-box/edge name. We need to apply this not only to the conclusion but also all formulas in the conditions:

% \[
%   \AxiomC{$\Gamma \vdash X$}
%   \RightLabel{\scriptsize(Rename)}
%   \UnaryInfC{$\rn(\Gamma) \vdash \rn(X)$}
%   \DisplayProof
% \]

% To have a model of $(\Sigma, E)$ in a compact closed symmetric monoidal category $C$ we need to assign morphisms in $C$ to each concrete diagram. Since all diagrams are built up from the generators we need only assign morphisms to the generators. If !-boxes occur in generators then we need a whole family of morphisms in $C$. For example, $\phi_{\+a \rexp{\<b}^B}$ requires a family of morphisms indexed by $i\in\mathbb{N}$ where $\phi_i$ is a morphism from the identity object $I$ to the object $X\otimes (X^*)^i$.

% \begin{remark}
%   In our graphical language we keep track of free edges via naming whereas in a category morphism inputs and outputs are ordered. Hence to go from a diagram to a morphism we must impose an order on the edgenames. Which order we choose is unimportant as swapping the order of two edge names is equivalent to applying a symmetry morphism swapping their corresponding morphism outputs. For this paper we will assume that we have a total order on the set $\edgenames$ of edgenames and hence that the objects of morphisms are ordered in correspondence with edgename order.
% \end{remark}

% A different approach to studying models is in an existing abstract tensor system, in the style of Penrose. In~\cite{KissingerATS} there is a proof that these two points of view (categorical vs. ATS) are equivalent, up to the use of order vs. names to distinguish free edges.

\begin{definition}
  An assignment from $\Sigma$ to the category $C$ is a map assigning a morphism to each concrete instance of a generator in $\Sigma$. The edges being ordered as they appear clockwise around the node.
\end{definition}

An assignment from $\Sigma$ to $C$ then naturally extends to an assignment mapping $\sgraphterms$ to morphisms of $C$ by combining the generating morphisms with $\eta_X$, $\epsilon_X$, identity morphisms and swap morphisms. Now that we have a unique morphism to represent each diagram we can check whether any two diagrams are equal under this assignment. We say a diagram equation holds under the assignment if the two diagrams are mapped to the same morphism.

\begin{definition}
  A \textit{model}, $\mathcal{M}$, of $(\Sigma,E)$ in the category $C$ is an assignment from $\Sigma$ to $C$ such that all (concrete instances of) equations in $E$ hold.
\end{definition}

A semantics for concrete graph equations can now be defined which takes concrete equations to $\{\true,\false\}$ (True vs False).

\begin{definition}
  If $G$ and $H$ are concrete graphs then
  \[\sem{G=H}:=\begin{cases}
    \true & G=H \text{ holds under any model of } (\Sigma,E). \\
    \false & \text{otherwise}
  \end{cases}\]
\end{definition}

Recall that a !-tensor equation $G=H$ with one free !-box $B$ represents a family of concrete graphs, in this case $\{\Kill_B\circ\Exp_B^n(G=H):n\in\mathbb{N}\}$, each of which can now be assigned a truth value through $\sem{-}$. Hence the semantics for $G=H$ becomes a map from each concrete instantiation of the !-box $B$ to truth values and the semantics for $\forall B.(G=H)$ should assert that each instantiation maps to truth. This notion can be extended to work for general !-tensor equations where $\sem{G=H}$ maps the instantiations of $\Boxes(G=H)$ to $\{\true,\false\}$.



\subsection{Semantics}\label{sub:semantics}

As suggested previously we wish to define a semantics which for any formula, $X$, assigns a map from $\inst{X}$ to $\{\true,\false\}$. 

\begin{definition}
  For a formula $X$, the \textit{semantics} of $X$, $\sem{X} : \inst{X}\mapsto\{\true,\false\}$ is defined recursively by:
  \begin{itemize}
    \item $\sem{G=H}(i) := \sem{i(G)=i(H)}$
    \item $\sem{X\wedge Y}(i) := \sem{X}(i|_X) \wedge \sem{Y}(i|_Y)$
    \item $\sem{X\rightarrow Y}(i) := \sem{X}(i|_X) \rightarrow \sem{Y}(i|_Y)$
    \item $\sem{\quant{A} X}(i) := \bigwedge_{j\in \inst{\downset{A}}} \sem{X}(i\circ j)$
  \end{itemize}
\end{definition}

Note that in the last case we have used the fact that operations in $\inst{\downset{A}}$ extend an instantiation of $\Boxes(\quant{A} X)$ to an instantiation of $\Boxes(X)$.
% Also in the middle two cases the instantiation $i$ may contain operations on !-boxes which do not occur in $X$ hence we write $i|X$ for the restriction of $i$ to operations on !-boxes in $X$.

% \begin{definition}
%   To save space and improve readability we will use the shorthand notation $\semi{X}$ rather than $\sem{X}(i|_X)$ when $i$ is an instantiation of a !-box structure containing $\Boxes(X)$ as a component.
% \end{definition}


We now present an example diagrammatic theory and use !-box induction to prove a generalised version of one of its axioms. We will look at a bialgebra, which can be built up from a monoid (white nodes) and a comonoid (grey nodes) with some additional interaction rules:

Monoid: \[\Sigma_{M} = \left\{\whitemult, \whiteunit \right\}\qquad E_{M} = \left\{\tikzfig{unit-law},\quad \tikzfig{assoc},\quad \tikzfig{mult-comm}\right\}\]

Comonoid: \[\Sigma_{C} = \left\{\graycomult, \graycounit \right\}\qquad E_{C} = \left\{\tikzfig{counit-law},\quad \tikzfig{coassoc},\quad \tikzfig{comult-comm}\right\}\]

Bialgebra: \[\Sigma_{B} = \Sigma_{M}\cup\Sigma_{C}\qquad E_{B} = E_{M}\cup E_{C}\cup\left\{ \tikzfig{bialg-dist-laws} \right\}\]

We can define an arbitrary arity white node to replace tree like structures of white nodes (and similarly for cotrees of grey nodes):



Note that since we have commutativity and associativity we don't need to worry about what order the edges enter our new node or which direction the tree associates. 

Now we can replace the monoid and comonoid theories with new arbitrary arity versions:

Monoid: \[\Sigma'_{M} = \left\{\tikzfig{mult_box} \right\}\qquad E'_{M} = \left\{\tikzfig{mult_spider},\quad\tikzfig{whitespider_elim}\right\}\]

Comonoid: \[\Sigma'_{C} = \left\{\tikzfig{comult_box} \right\}\qquad E'_{C} = \left\{\tikzfig{comult_spider},\quad\tikzfig{grayspider_elim}\right\}\]
